ReNeLiB: Real-time Neural Listening Behavior Generation for Socially Interactive Agents

Flexible and natural nonverbal reactions to human behavior remain a challenge for socially interactive agents (SIAs) that are predominantly animated using hand-crafted rules. While recently proposed machine learning based approaches to conversational behavior generation are a promising way to address this challenge, they have not yet been employed in SIAs. The primary reason for this is the lack of a software toolkit integrating such approaches with SIA frameworks that conforms to the challenging real-time requirements of human-agent interaction scenarios. In our work, we for the first time present such a toolkit consisting of three main components: (1) real-time feature extraction capturing multi-modal social cues from the user; (2) behavior generation based on a recent state-of-the-art neural network approach; (3) visualization of the generated behavior supporting both FLAME-based and Apple ARKit-based interactive agents. We comprehensively evaluate the real-time performance of the whole framework and its components. In addition, we introduce pre-trained behavioral generation models derived from psychotherapy sessions for domain-specific listening behaviors. Our software toolkit, pivotal for deploying and assessing SIAs' listening behavior in real-time, is publicly available. Resources, including code, behavioural multi-modal features extracted from therapeutic interactions, are hosted at https://daksitha.github.io/ReNeLib

==> 06_Results.tex <==
\section{Results}
\label{restuls}
Our real-time framework was evaluated on a machine equipped with an i9-13900KF processor (24 cores, 3.0 GHz - 5.8 GHz Turbo), RTX4090 GPU, and running Ubuntu 22.04, employing the modules depicted by solid black arrows in Fig.~\ref{fig:frameworkOverview}. Utilizing a MS Kinect v2‚ camera with 30 fps and 24 fps and a microphone array comprising four microphones processing 16-bit audio at a 16 kHz sampling rate, we configured the system with $T_{audio}=0.5$s for capturing the audio signal and then processing Mel frequencies. We set $T_{video}=1$s for capturing the audio stream and process and publishing a batch of 30 and 24 images after every second using the FLAME extractor. The audio Mel frequencies were re-sampled at $4 \times F_{fps} \times T_{audio}$ fps to facilitate unified feature processing. In our evaluation scenario illustrated in Fig.~\ref{fig:realtime}, where $F_{fps}=30$ and 
 $M_{fps}=120$, similarly for 24 fps scenario. The Mel frequency module published data to the multimodal data queue in the behavior generation module at 0.5s intervals whereas FLAME features at 1s intervals. By adjusting the $T_{video}$ and $T_{audio}$ lengths of the processing data for each extractor module, we can identify a data throughput bottleneck if the processing time exceeds the capture time, as demonstrated by the extractor plots shown in Fig.~\ref{fig:realtime}.

As the feature queues began filling at the incoming frame rate determined by each feature extractor module, the behavior prediction module processed data with a sliding window, initially using empty feature queues. This approach enabled the generation of behavior irrespective of the incoming frame rates from the extractor modules while synchronizing multimodal data with computed timestamps. Concurrently, the time required by the LiveFLAME and web-based VuppetMaster animation modules to animate the interactive agent is presented in Fig.~\ref{fig:animationtime}. The obtained results underscore the framework's capacity to sustain low latency and process data effectively, emphasizing its suitability for real-time applications in interactive contexts.



%Our real-time framework was evaluated on a machine equipped with an i9-13900KF processor (24 cores, 3.0 GHz - 5.8 GHz Turbo), RTX4090 GPU, running Ubuntu 22.04, employing thick black arrow modules shown in  \ref{fig:frameworkOverview}. Utilizing a Kinect camera with 30 fps and a microphone array consisting of four microphones processing 16-bit audio at a 16 kHz sampling rate, we configured the system with $T_{audio}=0.5$s for capturing and processing Mel frequencies every 0.5s and $T_{video}=1$s for processing and publishing a batch of 30 images per second using the FLAME extractor. The audio Mel frequencies were re-sampled at $4 \times F_{fps} \times T_{audio} $ fps to facilitate unified feature processing.  In our evaluation scenario illustrated in Fig \ref{fig:realtime}, $F_{fps}=30$ and the resulting $M_{fps}=120$ though the Mel frequency module stream data to multimodal data queue in behaviour generation modle at a faster rate than the FLAME features. As the feature queues started filling at the incoming frame rate determined by each feature extractor module, the behaviour prediction module process data with a sliding window, while inintialised with a empty feature queues. This way it can generate behaviour regardless of the incoming frame rates from extractor module while synchronising with timestamps. Concurrently, the time required by each animation module LiveFLAME and web-based VuppetMaster to animate the interactive agent is presented in Fig \ref{fig:animationtime}. The obtained results underscore the framework's capacity to sustain low latency and process data effectively, emphasizing its aptness for real-time applications in interactive contexts.



%The performance of our real-time framework was assessed on a machine equipped with an i9-13900KF processor (24 cores, 3.0 GHz - 5.8 GHz Turbo), GTX 4090 GPU. Modules outlined with a thick black arrow in fig \ref{fig:frameworkOverview} were thoroughly tested, utilizing a Kinect 30 fps camera and a microphone array with four microphones processing 16-bit audio at a sampling rate of 16 kHz. The configuration was set to $T_{audio}=0.5$s for capturing and processing Mel frequencies every 0.5s and $T_{video}=1$s for the FLAME extractor to process a batch of 30 images and publish every second. The audio Mel frequencies were resampled at $4 \times 30$ fps to enable unified processing of the features.

%The feature queues began filling at the incoming frame rate specified by each feature extractor module. The evaluation results for real-time data processing are illustrated in Fig \ref{fig:realtime}, while the time taken by each animation module to animate the interactive agent is depicted in Fig \ref{fig:animationtime}. These findings demonstrate the framework's ability to maintain low latency and process data efficiently, highlighting its suitability for real-time applications in interactive scenarios.

==> alt-text.tex <==
Figure 1: \Description[A framework that enables interactive virtual agents to dynamically adapt to user behavior through the analysis of multimodal social cues]{Experience ReNeLiB: A framework transforming human-webcam interactions through 3D motion and Mel frequency analysis, enabling interactive virtual agents to adapt to user behavior based on multimodal social cues}
Figure 2: \Description[The framework with publisher-subscriber design for real-time behavior. Supports online/offline modes and local or sensor data. Solid arrows show evaluated modules.]{Overview of the real-time interactive framework modules, utilizing a publisher-subscriber pattern to enable real-time listener behavior. The framework supports both online and offline modes, allowing for feature extraction from sensors or streaming from locally saved files. The solid arrows represent the modules used in our evaluation.}
Figure 3: \Description[VQ-VAE training process]{VQ-VAE training process}
Figure 4: \Description[Predictor training process]{Predictor training process}
Figure 5: \Description[FLAME to ARKit expression mapper]{FLAME to ARKit expression mapper}
Figure 6: \Description[Network latency plot for each framework module for different frame rates]{Network latency plot for each framework module for different frame rates}
